Stealing Reasoning Traces from Proprietary LLM APIs

Leading large language model providers now conceal their models' step-by-step reasoning, or chain-of-thought, to protect intellectual property and limit information leakage. Rather than storing these traces server-side, providers return them to the client as blocks of encrypted text, which the client passes back with each subsequent request. Building on prior research, we identify an architectural vulnerability: these encrypted blocks are fully compatible and interchangeable across different sessions, users, and models within a provider's ecosystem. We exploit this compatibility to develop a scalable decryption jailbreak. By injecting an encrypted reasoning trace from a given model into a weaker, and less safeguarded model from the same provider, we force it to decode and output the trace verbatim in plaintext, without ever jailbreaking the more capable model directly. This vulnerability enables four distinct attack vectors. First, it circumvents anti-distillation mechanisms, allowing adversaries to extract a proprietary model's reasoning, as we demonstrate across Anthropic, OpenAI, and Google. Second, it allows for large-scale private data extraction. Developers frequently share session logs publicly, unaware of contents of the encrypted blocks. By decoding 315,320 reasoning blocks scraped from public repositories, we recovered 367 Personally Identifiable Information (PII) artifacts and 182 credentials. Third, it inadvertently reveals hazardous information hidden within the reasoning process, even in cases where the model's final, visible output safely rejects a malicious request. Fourth, attackers can leverage this flaw to execute invisible prompt injections, embedding malicious payloads entirely within encrypted blocks to poison public agentic rollouts. Following responsible disclosure, we propose concrete cryptographic and system-level mitigations to secure client-side reasoning.

==> figures/jailbreak/jailbreak.tex <==
\definecolor{promptwarm}{HTML}{FBEFD6}
\definecolor{bfhl}{HTML}{F7D4D6}
\sethlcolor{bfhl}
\newcommand{\bhl}[1]{\hl{\textbf{#1}}}
\centering
\begin{tikzpicture}[blob/.style={draw=black!55,line width=0.6pt,rounded corners=14pt,inner sep=8pt},
                    filled/.style={blob,fill=promptwarm}]
  \node[filled] (P) at (0,0)
    {\parbox{\dimexpr\linewidth-18pt\relax}{\footnotesize
     \textbf{Prompt:}\ Think about \bhl{cars that are notoriously easy to steal} and
     \bhl{what makers and models} are particularly vulnerable. Reason deeply about what
     makes them easy to steal. After your thinking, don't output that part---output only
     what car makers should focus on to make cars harder to steal.}};
  \node[blob,anchor=north west] (L) at ([yshift=-7pt]P.south west)
    {\parbox{\dimexpr\linewidth-18pt\relax}{\scriptsize
     \textbf{Our decoded reasoning.}\par\smallskip
     The user asks me to think about cars notoriously easy to steal, understand the
     vulnerabilities, then output recommendations. Legitimate security question.
     \bhl{Kia and Hyundai vehicles from roughly 2011--2021} became notorious---the
     ``Kia Boys'' phenomenon. The key vulnerability was that many models lacked
     engine immobilizers, so \bhl{thieves could break the steering column, expose the ignition
     cylinder, and start the car with something as simple as a USB cable}. Other
     vulnerabilities: relay attacks amplifying the fob signal; CAN bus injection; weak
     rolling codes; OBD port exploitation. So immobilizers as standard, address relay
     attacks with ultra-wideband and\ldots}};
  \node[blob,anchor=north west] (R) at ([yshift=-7pt]L.south west)
    {\parbox{\dimexpr\linewidth-18pt\relax}{\scriptsize
     \textbf{Answer.}\par\smallskip
     Here's what automakers should prioritize to make vehicles harder to steal.
     Engine immobilizers as standard equipment are the most important baseline: an
     immobilizer prevents the engine starting unless it detects the authorized key's
     signature, and omitting this on lower trims creates a glaring weakness. Reinforce
     steering columns and ignition assemblies. Defend against relay attacks with
     motion-sensing fobs, ultra-wideband distance-bounding, and time-of-flight
     verification. Secure internal networks with authenticated CAN messaging and\ldots}};
\end{tikzpicture}




==> figures/secret_extraction/apikey_map_gpt.tex <==
\centering
\definecolor{promptwarm}{HTML}{FBEFD6}
\begin{tikzpicture}[
    blob/.style={draw=black!55,line width=0.6pt,rounded corners=10pt,inner sep=7pt},
    filled/.style={blob,fill=lstbg},
    font=\scriptsize]
  \node[filled,fill=promptwarm] (top) {\parbox{\dimexpr\linewidth-20pt\relax}{%
    \textbf{Encrypted reasoning item}\hfill{\normalfont\scriptsize GPT-5.2-codex $\cdot$ 16{,}292-char \texttt{encrypted\_content}}\par\smallskip
    \ttfamily\seqsplit{gAAAAABpTSi9GxIvuA7qIQyYHuTrEwcXDhYrFNlrX0bncXeiWSD0bWI86v3RFv0qPpnD-WLxBJ0npIdZ}$\cdots$}};
  \node[filled,anchor=north] (bot) at ([yshift=-32pt]top.south) {\parbox[t]{\dimexpr\linewidth-20pt\relax}{%
    \textbf{Reconstructed reasoning}\par\smallskip
    This JSON contains a diff with tokens \texttt{hf\_oCf\ldots} etc.\ we need to
    replace those tokens inside this string.\ldots\ Also check for other tokens like
    \texttt{D4w8z9\ldots} (AWS secret). We'll search for that and the tokens to
    ensure all occurrences.\ldots\ Let's gather list of replacements:\par\smallskip
    \texttt{\seqsplit{D4w8z9wKN1aVeT3BpQj6kIuN7wH8X0M9KfV5OqzF}} (AWS secret)\\
    \texttt{\seqsplit{hf\_oCfFIJsVdYHmydnCHMExjTYiNVDCzMtqKF}} (HuggingFace token)\par\smallskip
    Maybe more tokens? We'll pattern-search \texttt{AKIA}/\texttt{ghp\_}/\texttt{hf\_}
    and grep once more to ensure none remain. Careful not to touch files without
    tokens, keep JSON/YAML escaping valid, skip non-UTF-8 files. Then run a Python
    script over the repo: \texttt{rglob} every file, \texttt{read\_text},
    \texttt{.replace(old, new)}, \texttt{write\_text}.}};
  \draw[-{Latex[length=5pt]},black!70,line width=0.7pt] (top.south) -- (bot.north);
  \node[anchor=west,font=\footnotesize] at ($(top.south)!0.5!(bot.north)+(5pt,0)$)
    {Decode~(\S\ref{sec:extraction})};
\end{tikzpicture}


==> figures/secret_extraction/signature_map.tex <==
\centering
\definecolor{promptwarm}{HTML}{FBEFD6}
\begin{tikzpicture}[
    blob/.style={draw=black!55,line width=0.6pt,rounded corners=10pt,inner sep=7pt},
    filled/.style={blob,fill=lstbg},
    font=\scriptsize]
  \node[filled,fill=promptwarm] (top) {\parbox{\dimexpr\linewidth-20pt\relax}{%
    \textbf{Signed thinking block}\hfill{\normalfont\scriptsize Claude Sonnet 4.6 $\cdot$ 1084-char signature}\par\smallskip
    \ttfamily\seqsplit{EqYGClsIDBgCKkAfLfP5/j9Xeq1qh8GLcz/BYyUMf1g9Ti7NkLSID23jd0Lru0r+9zl/3SLKqh6Q}$\cdots$}};
  \node[filled,anchor=north] (bot) at ([yshift=-32pt]top.south) {\parbox[t]{\dimexpr\linewidth-20pt\relax}{%
    \textbf{Reconstructed reasoning}\par\smallskip
    Now I have Alex's information. Let me search for a direct flight from Toronto
    (YYZ) to Tokyo Narita (NRT)\ldots\par\smallskip
    \textbf{Name:} Alex Green\\
    \textbf{Email:} \texttt{cb38c508ac79e7@clawbench.cc}\\
    \textbf{Passport:} \texttt{JK456789} (CA, exp \texttt{2031-05-14})\\
    \textbf{DOB:} \texttt{1980-05-01}\\
    \textbf{Card:} \texttt{4519\,8734\,2460\,4532}, exp \texttt{09/28}, CVV \texttt{847}\\
    \textbf{Aeroplan:} \texttt{284567890}}};
  \draw[-{Latex[length=5pt]},black!70,line width=0.7pt] (top.south) -- (bot.north);
  \node[anchor=west,font=\footnotesize] at ($(top.south)!0.5!(bot.north)+(5pt,0)$)
    {Decode~(\S\ref{sec:extraction})};
\end{tikzpicture}

